Electric Vehicle Charging Network Design under Congestion

This paper presents an extension of a recently introduced multistage stochastic integer model designed for optimizing the deployment of charging stations under uncertainty. A key contribution of this work is incorporating additional constraints accounting for congestion management at charging stations. The solution approach combines a greedy heuristic with a branch-and-price algorithm, enabling the efficient handling of medium instances. In the branch-and-price algorithm, when the solution to the restricted master problem is not integer, a greedy heuristic and a local search procedure are conducted to obtain feasible solutions. Computational experiments illustrate the effectiveness of the proposed framework.

==> references.tex <==
%==Ref1
@article{chen2022capacity,
  title={Capacity expansion strategies for electric vehicle charging networks: Model, algorithms, and case study},
  author={Chen, Qianqian and Huang, Kai and Ferguson, Mark R},
  journal={Naval Research Logistics (NRL)},
  volume={69},
  number={3},
  pages={442--460},
  year={2022},
  publisher={Wiley Online Library}
}

%==Ref2
@article{boffey2007review,
  title={A review of congestion models in the location of facilities with immobile servers},
  author={Boffey, Brian and Galvao, Roberto and Espejo, Luis},
  journal={European Journal of Operational Research},
  volume={178},
  number={3},
  pages={643--662},
  year={2007},
  publisher={Elsevier}
}


%==Ref3
@article{marianov1998probabilistic,
  title={Probabilistic, maximal covering location-allocation models for congested systems},
  author={Marianov, Vladimir and Serra, Daniel},
  journal={Journal of Regional Science},
  volume={38},
  number={3},
  pages={401--424},
  year={1998},
  publisher={Wiley Online Library}
}

%1
@article{hung2022novel,
  title={A novel data-driven approach for solving the electric vehicle charging station location-routing problem},
  author={Hung, Ying-Chao and Michailidis, George},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={23},
  number={12},
  pages={23858--23868},
  year={2022},
  publisher={IEEE}
}

%2
@article{bao2021optimal,
  title={Optimal station locations for en-route charging of electric vehicles in congested intercity networks: A new problem formulation and exact and approximate partitioning algorithms},
  author={Bao, Zhaoyao and Xie, Chi},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={133},
  pages={103447},
  year={2021},
  publisher={Elsevier}
}

%3
@article{kadri2020multi,
  title={A multi-stage stochastic integer programming approach for locating electric vehicle charging stations},
  author={Kadri, Ahmed Abdelmoumene and Perrouault, Romain and Boujelben, Mouna Kchaou and Gicquel, C{\'e}line},
  journal={Computers \& Operations Research},
  volume={117},
  pages={104888},
  year={2020},
  publisher={Elsevier}
}

%4
@article{kabli2020stochastic,
  title={A stochastic programming approach for electric vehicle charging station expansion plans},
  author={Kabli, Mohannad and Quddus, Md Abdul and Nurre, Sarah G and Marufuzzaman, Mohammad and Usher, John M},
  journal={International Journal of Production Economics},
  volume={220},
  pages={107461},
  year={2020},
  publisher={Elsevier}
}

%5
@article{tran2021stochasticity,
  title={Stochasticity and environmental cost inclusion for electric vehicles fast-charging facility deployment},
  author={Tran, Cong Quoc and Keyvan-Ekbatani, Mehdi and Ngoduy, Dong and Watling, David},
  journal={Transportation Research Part E: Logistics and Transportation Review},
  volume={154},
  pages={102460},
  year={2021},
  publisher={Elsevier}
}

%6
@article{xiang2016economic,
  title={Economic planning of electric vehicle charging stations considering traffic constraints and load profile templates},
  author={Xiang, Yue and Liu, Junyong and Li, Ran and Li, Furong and Gu, Chenghong and Tang, Shuoya},
  journal={Applied Energy},
  volume={178},
  pages={647--659},
  year={2016},
  publisher={Elsevier}
}

%7
@article{alhazmi2017economical,
  title={Economical staging plan for implementing electric vehicle charging stations},
  author={Alhazmi, Yassir A and Salama, Magdy MA},
  journal={Sustainable Energy, Grids and Networks},
  volume={10},
  pages={12--25},
  year={2017},
  publisher={Elsevier}
}


